DisCoveR: Accurate & Efficient Discovery of Declarative Process Models

Declarative process modeling formalisms - which capture high-level process constraints - have seen growing interest, especially for modeling flexible processes. This paper presents DisCoveR, an extremely efficient and accurate declarative miner for learning Dynamic Condition Response (DCR) Graphs from event logs. We precisely formalize the algorithm, describe a highly efficient bit vector implementation and rigorously evaluate performance against two other declarative miners, representing the state-of-the-art in Declare and DCR Graphs mining. DisCoveR outperforms each of these w.r.t. a binary classification task, achieving an average accuracy of 96.2% in the Process Discovery Contest 2019. Due to its linear time complexity, DisCoveR also achieves run-times 1-2 orders of magnitude below its declarative counterparts. Finally, we show how the miner has been integrated in a state-of-the-art declarative process modeling framework as a model recommendation tool, discuss how discovery can play an integral part of the modeling task and report on how the integration has improved the modeling experience of end-users.

==> aggregate_confusion_matrix.tex <==
\begin{table*}[h!]
\begin{tabularx}{\textwidth}{ l | l | c c | c c | c c}
												&						& \multicolumn{6}{c}{\textbf{\textsc{Observed}}}\\
\midrule
												&						& \multicolumn{2}{c}{DisCoveR} 			& \multicolumn{2}{c}{Debois}			& \multicolumn{2}{c}{MINERful} \\
\midrule
												&						& \textsc{Legal}  	& \textsc{Illegal} 	& \textsc{Legal}  	& \textsc{Illegal} 	& \textsc{Legal}  	& \textsc{Illegal} \\
\multirow{2}{*}{\textbf{\textsc{Predicted}}} 	& \textsc{Legal}		& 448				& 30 				& -					& -					& -					& -			\\
												& \textsc{Illegal} 		& 5					& 417	 			& -					& -					& -					& - \\			
\end{tabularx}
\label{tab:results_confusion_aggregate}
\caption{Aggregate confusion matrices}
\end{table*}

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}

==> ecoknow.tex <==
The EcoKnow (Effective, co-created and compliant adaptive case management for Knowledge workers) project is a four year, inter-disciplinary research project initiated September 2017. The scientific basis of the project spans from field studies of case management and computer supported cooperative work, over development of workflow technologies based on formal declarative models to machine learning and studies of the understandability of modelling notations.

The aim provide technologies for flexible, agile and transparent digitalization of governmental case management process that at the same time increase the quality with respect to compliance and equal treatment of citizens with respect to the law and reduce wasteful delays in case management. 

A key hypothesis of the project is that the declarative DCR Graph modelling notation supports an agile, incremental digitalisation of workflows that can be understood, developed and maintained locally in governmental institutions instead of relying on vendors of case management solutions encoding the law and other rules to be followed in the solutions.

Being now half way through the project, the hypothesis has been partially validated. 
The DCR technology has successfully been embedded in commercial case management systems used widely in both local and central government institutions in Denmark. The technology has also made available as part of an open source case management tool, the Open Case Manager, which is now used in the daily case management in a Danish municipality taking part of the project. 

To support the local development and maintenance of the declarative DCR models, several modelling tools have been developed and understandability studies have been carried out. 



==> regularization.tex <==
\subsection{Regularization}
\label{sec:regularization}



==> related_work_flaviaspaper.tex <==
\textbf{COB: This section may have become too extensive. Let me know if it needs to be condensed or if some material is irrelevant. (Or just go ahead and remove it.)}

The challenges of merging event-related data from disparate and incongruous sources into a coherent event log are well known \cite{bose2013wanna}. Quality issues are sufficiently prevalent to have spurred work on the formalization of event log imperfection patterns to facilitate the identification and remedy of commonly recurring shortcomings \cite{suriadi2017event}. Additional challenges are posed by the increasing focus on event \emph{streams}, rather than static, complete event logs \cite{van2018event}. 

Process mining centers around \emph{events}, which are often not given a central role in traditional data schemas, and sometimes produced only as a by-product. Correlating events to form process instances is not always straightforward, and often system specific. In \cite{de2016process} the authors use database redo logs to do so in a system-independent manner. Events may even need to be extracted from auxiliary sources lacking a common case identifier \cite{mannhardt2014extending} or even buried in digital communications \cite{di2013mining}.

One application of conformance checking is to the data cleaning and event log preparation procedure itself \cite{wang2015cleaning,de2012aligning,de2015alignment,rogge2013repairing}. But the primary aim of conformance checking tends to be: determining the degree of adherence to business rules and regulations and detecting past, current, or potential violations; and conversely, assessing whether a model accurately reflects reality. A distinction can be drawn between \emph{backward} conformance checking, which aims to identify and localize violations that have happened, and \emph{forward} compliance checking which focuses on the design of compliant processes and prescription of future courses of action during process execution to ensure compliance \cite{diagnostic2013}.

%A number of conformance checking approaches exist, depending on the modeling formalism and the chosen conformance metric. 
The simplest formulation of conformance checking is that of trace- or case-level fitness, i.e. whether entire traces are permitted by a model or not \cite{adriansyah2010towards}. This is used as the basis for the \emph{Parsing Measure} of model quality in \cite{weijters2006process}. As the authors note, this measure glosses over important details in the degree and nature of model-log inconsistency. Instead, measures of violations at the level of the individual event are needed, not only for accuracy, but to assist in locating potential areas for improvement \cite{goedertier2007process,goedertier2009robust}.

A prevalent approach to quantifying the \emph{degree} of model-log incongruity is that of alignment, which defines a distance function\footnote{Not to be confused with a proper \emph{metric} fulfilling the axioms of non-negativity, identity of indiscernibles, symmetry and the triangle inequality.} between a trace and a model based on the minimum number of extra ``moves'' that must be inserted into either trace or model to replay the trace and reach an accepting state in the model \cite{adriansyah2012alignment,van2012replaying}. Any trace replayable on a model without modification will have an alignment distance of zero. Alignment can also capture the severity of incongruities by assigning costs to individual edits \cite{de2016computing}. Alignment based approaches are not formalism-specific and have been applied to declarative models in \cite{de2016computing,de2012aligning,de2015alignment}.

Some of the most formalism-specific metrics are token-based measures for Petri nets (specifically workflow nets) based on the number of tokens that were missing in the model when replaying a trace/log, and the number remaining in the model after replay, relative to the total number of tokens consumed and produced overall \cite{rozinat2008conformance}. In \cite{diagnostic2013}, a conformance checking technique based on data-aware Petri nets is presented which handles both contol-flow and timing constraints by modeling time as a data attribute. Some declarative models can be translated into workflows nets, and are thereby amenable to token-based metrics. See \cite{declare2rinets} for an overview of translations from Declare constraints to Petri nets with reset and inhibitor arcs.

One important nuance afforded by the declarative approach is the ability to perform \emph{runtime verification} by distinguishing between constraints being \emph{permanently} satisfied/violated and \emph{possibly} violated \cite{lookingintofuture}. This perspective lends itself naturally, not only to prediction, but to prescription of best courses of action.

Conformance checking for declarative models varies depending on the specific formalism, though translation to finite state automata is common. Temporal logics, such as linear temporal logic (LTL), computational tree logic (CTL), CTL*, event calculus \cite{cicekli2006formalizing} form the foundation of much declarative process modeling, with Declare being a canonical example originally formulated as set of templates based on LTL and since extended (see below). Stochastic process algebras such as PEPA are similar to other declarative languages in their compositional nature and amenability to qualitative analysis while facilitating quantitative analysis via translation to stochastic Markov models \cite{hillston2005process}.
%Not to be confused with LTL, linear logic is a resource oriented logic allowing for correct-by-design optimally concurrent process formulation.

Conformance checking of temporal logic based languages can be done via translation into a set of finite-state automata (FSA), (non-)deterministic FSA (NFA/DFA) in the case of constraints on finite traces, and B\"uchi automata in the infinite case \cite{DeGiacomo:2014,metaconstraintsLTLLDL}. The conjunctive nature of these logics means that the product of corresponding automata is sufficient to capture any potential interplay. A non-accepting terminal state in the the resulting automaton translates as a permanent violation of the model, for example. Alternatively, rewrite rules can be employed such that replaying an event results in a new set of formulae representing the constraints to be satisfied in the remaining execution of the process \cite{Basin2015}.

Recently, extensions to such \emph{propositional} temporal logics incorporating timing and data have seen growing interest. Going beyond simple ordering constraints, these logics allow specification of constraints w.r.t. absolute and relative time and quantified statements about the world. 
%Modifying slightly an example from \cite{fu2015computational}, ``the vehicle must enter region $A$ with the first 5 minutes, and subsequently enter region $B$ within 3 minutes of entering region $A$''.

Metric (interval) temporal logic (MTL/MITL) is one such logic, variants of which differ in terms of semantics: point-based vs. interval-based; and time representation: dense vs. countable \cite{ouaknine2008some}.  Some of these fragments can be checked via mapping to LTL \cite{hustadt2017theorem} or via timed automata \cite{lookingintofuture}, allowing for time-based runtime verification and operational support \cite{Basin2018}. 

Metric \emph{first-order} temporal logic (MFOTL) extends MTL with first order formulae quantified over infinite domains \cite{timedmultiperspective}, allowing constraints stating that first-order statements be true at a given time or interval. Conformance checking for MFOTL is in general undecidable, but for a subset of constraints based on Declare, algorithms are presented in \cite{burattin2016}.

DCR graphs differs from the temporal logics discussed above, in particular in its non-monotonic properties \cite{}\todo{@Tijs}. That is, adding a rule does not necessarily further restrict the behavior permitted by a model - it may indeed increase it. Nonetheless, DCR constraints can also be converted to (B\"uchi) automata for conformance checking \cite{thomasrao2010}. 
